Toward Moir\'e-Free and Detail-Preserving Demosaicking

3D convolutions are commonly employed by demosaicking neural models, in the same way as solving other image restoration problems. Counter-intuitively, we show that 3D convolutions implicitly impede the RGB color spectra from exchanging complementary information, resulting in spectral-inconsistent inference of the local spatial high frequency components. As a consequence, shallow 3D convolution networks suffer the Moir\'e artifacts, but deep 3D convolutions cause over-smoothness. We analyze the fundamental difference between demosaicking and other problems that predict lost pixels between available ones (e.g., super-resolution reconstruction), and present the underlying reasons for the confliction between Moir\'e-free and detail-preserving. From the new perspective, our work decouples the common standard convolution procedure to spectral and spatial feature aggregations, which allow strengthening global communication in the spectral dimension while respecting local contrast in the spatial dimension. We apply our demosaicking model to two tasks: Joint Demosaicking-Denoising and Independently Demosaicking. In both applications, our model substantially alleviates artifacts such as Moir\'e and over-smoothness at similar or lower computational cost to currently top-performing models, as validated by diverse evaluations. Source code will be released along with paper publication.

==> introduction.tex <==
\section{Introduction}
Demosaicking is to reconstruct RGB images from raw Color Filter Array (CFA, usually Bayer) images, which sample the RGB signals at different pixels. The missing low frequency component at each pixel must be inferred from intra-spectral information, as the RGB color representation is an orthogonal system. In contrast, to estimate the missing high frequency components sharply and cleanly, a demosaicking algorithm must explore the inter-spectral information, because: 1) the intra-spectral samples are sparse, hence insufficient to reflect the true distribution of the underlying signal; 2) if the high frequencies of the missing spectra are estimated inconsistently with the captured spectrum at a pixel, the inconsistency would cause Moir\'{e} and false color artifacts \cite{szeliski2010}. Although such artifacts can be alleviated by high frequency smoothing, image details would be blurred as a side effect. 

For accurate detail reconstruction, a myriad of demosaicking models have been proposed to investigate the spectral-spatial correlation of the CFA samples. Commonly, they boil down to combining high-order filtering activation maps of each spectra, where the filters and the combination scheme may be designed by mathematical priors (e.g., \cite{HA96, HQLI04, MLRI16, NiuTIP2019, ni2020color}), or may be learned from data (e.g., \cite{MSR2014}, \cite{LDSR14}, \cite{DDR16}, \cite{MNN14}). Recently, Convolutional Neural Networks have been intensively investigated for combined spectral-spatial representation (\cite{2016DJDD, MDFCN18, CAS18, chen2021Wild, 2Stage17, 3Stage18, 2018kokkinos, liu2020SG, 2020NTSDCN, yan2019channel, elgendy2021low, liu2020SG, 2021xing, zhang2022deep, 2022mutual}). The inter-spectral correlation can be further explored by using the green information to guide the red and blue reconstruction  \cite{2Stage17, 3Stage18, liu2020SG, 2020NTSDCN}, or mutual guidance \cite{2022mutual}, or transforming the RGB restoration to color difference restoration \cite{yan2019channel, elgendy2021low}. As traditional convolution lacks spatial adaptiveness, Liu et al. proposed weighting the inter-spectral features by local contrast of the intermediately estimated green channel \cite{liu2020SG}; Zhang et al. proposed generating spatially varying convolution kernels from the CFA pattern \cite{zhang2022deep}. Although the Self-Attention mechanism \cite{2020ViT} is more spatially adaptive than 3D convolutions, it has been barely applied to demosaicking, due to its high memory consumption and heavy computation. 

Existing CNN-based models commonly employ 3D convolutions. This seems natural since 3D convolutions work well for other image interpolation problems, especially super-resolution reconstruction, which also predicts the in-between pixels. However, demosaicking is special. It is the unique image restoration problem that relies on the complementary information of all color spectra. 3D convolutions for demosaicking implicitly tie the spatial and spectral feature aggregation (see Sec.~\ref{sec:motivation} for in-depth analysis). Thus to deepen spectral information aggregation, spatial receptive field has to be expanded simultaneously, losing local spatial details. Moreover, as demosaicking allows no latency, the depth of 3D convolutions is generally refrained to avoid computation overload, leading to insufficient exchanging of information across the spectra. Therefore, using 3D convolutions for demosaicking would cause contradiction between maintaining global spectral consistency and local spatial anisotropic affinity, making Moire-free and detail-preserving exclusive. 

In view of this, we propose a new framework for Moire-free and detail-preserving demosaicking. We decouple the spectral and spatial aggregations, such that cross-spectral information communication is deepened and enhanced to secure spectral high frequency consistency, while the spatial representation is steered adaptively by local contrast. To achieve this goal without increasing computational cost, we adapt the MobileNetV3 building blocks and Self-Attention mechanism to our framework in an efficient fashion.  
% we notice that the 3D convolution is not well suited to Demosaicking (see Sec.~\ref{sec:motivation} for in-depth analysis). In this paper, we exploit the integration of Separable Convolution with Local Spatial Self-Attention for demosaicking. By decoupling 3D convolution to depth-wise (i.e., the spatial dimension) and point-wise (i.e., the spectral dimension) convolutions, it allows combining the filter activation maps in the spectral dimension more comprehensively than the spatial dimension. Thereby cross-spectral high frequency consistency is achieved without increasing the number of parameters or floating point operations. Furthermore, it enables using only five local Transformer units to achieve sharp and clean demosaicking.

% A fundamental difference between demosaicking and super-resolution is that, to be processed by convolutions, the CFA samples have to be reordered into spatial-spectral subbands first, such that each feature map contains samples of the same spectrum. That is, the feature dimension of the hidden feature tensors is actually the spectral dimension. Feature aggregation along the spectral dimension gets cross-spectra communication to share features and high-order statistics. However, 3D convolutions on hidden features bind the spectral and spatial convolutions together. As demosaicking has strict requirement on inference time, the depth of 3D convolutions should be refrained, which consequently limits information exchange across spectra, leading to Moir\'{e} or false color. 



% In this paper, to take advantage of Transformer for sharp and clean reconstruction without increasing the computational cost, we efficiently integrate MobileNet blocks with Local Transformer Attention in a U-net framework. Compared to plain 3D convolution, given the same budget on model complexity, MobileNet can extend deeper. Moreover, as MobileNet decouples 3D convolution to depth-wise (i.e., the spatial dimension) and point-wise (i.e., the spectral dimension) convolutions, it allows combining the filter activation maps in the spectral dimension more comprehensively than the spatial dimension. Thereby cross-spectral high frequency consistency is achieved without increasing the number of parameters or floating point operations. 
We extensively evaluate the proposed method for both joint demosaicking-denoising and pure demosaicking. Our model exhibits noticeable numerical and visual improvement over currently top preforming models, at comparable or lower computational cost, across a variety of benchmark datasets. 

%To summarize, our work makes the following contributions:
\textbf{Summary of contributions:}
 \begin{itemize}
    \item We unveil the deficiency of 3D convolutions for demosaicking, and analyze the underlying reasons for the deficiency.
    \item We provide a new perspective to formulate demosaicking, which we show requires \textit{global} aggregation of \textit{spectral} information and \textit{local} aggregation of \textit{spatial} information. This fact has been largely ignored in demosaicking literature.
    % \item We provide a new perspective to view demosaicking. We argue that Moir\'{e} is caused by the inconsistently inferred high frequency components across the RGB spectra. Instead of the commonly used 3D convolutions, depth-wise separable convolutions should be used for demosaicking for cross spectral consistency.
    \item We propose a new demosaicking framework, which strengthens cross-spectral information communication while sharpening spatial details, based on highly efficient separable convolutions and only a small number of Self-Attention units.
    \item Our model effectively circumvents demosaicking artifacts. It improves the state-of-the-art performance in either demosaicking or joint demosaicking-denoising tasks.
    
    % \item We propose a new demosaicking framework. We efficiently integrate Local Transformer Attention with sequential MobileNet Convolutions, to achieve detail-preserving and Moir\'{e}-free RGB image reconstruction.
    
    % \item We provide a novel spectral-spatial feature aggregation strategy. It respects spatial details while maintaining detail consistency across all spectra.
    % allows fusing features comprehensively across all spectra, then adaptively diffusing features along spatial edges.
    
    
 \end{itemize}

==> method.tex <==
\section{Proposed Method}
\begin{figure*}[htb]
\begin{center}
\includegraphics[width=1\linewidth]{figs/Network.png}
\end{center}
   \caption{The overall architecture of our model. The bayer image is first rearranged to four channels. The sub-branch generates intra-spectral features to guide the backbone mix inter-spectral features.}
\label{fig:Network}
\end{figure*}
Let $\mathbf{Y}$ be an RGB image captured by a tri-color sensor on a $2H\times 2W$ lattice $\mathcal{L}$. $\mathbf{Y}$ is composed of samples of the red, green and blue spectra $\mathbf{r}(\mathcal{L})$, $\mathbf{g}(\mathcal{L})$, and $\mathbf{b}(\mathcal{L})$. Let $\mathbf{X}$ be $\mathbf{Y}$'s corresponding CFA image captured by a Bayer sensor. Define subset $\mathcal{R}\in \mathcal{L}$ to collect the positions where the red values are captured, and define $\mathcal{G}$ and $\mathcal{B}$ similarly. $\mathcal{G}$ is further split to $\mathcal{G}_1$ and $\mathcal{G}_2$, which exclusively contain positions at the odd and even rows. We train a deep neural model $f_{\theta}(\mathbf{X})$ parameterized by $\theta$ to estimate $\mathbf{Y}$. 

We first describe the overall workflow of our model and explain the motivation for the design of each part, the details of which will then be elaborated in subsections.

\subsection{Overall Architecture}
Briefly, our end-to-end trainable model $f_{\theta}(\mathbf{X})$ adopts a hierarchical U-net encoder-decoder architecture.

Following the convention of demosaicking neural networks, our model first decomposes the input CFA image to four spatial-spectral subbands $\mathbf{r}(\mathcal{R})$, $\mathbf{g}(\mathcal{G}_1)$, $\mathbf{g}(\mathcal{G}_2)$, and $\mathbf{b}(\mathcal{B})$. 

We deploy a sequence of consecutive group convolutions to extract high-dimensional representations from each spatial-spectral subband. The base level intra-spectrum feature tensors are further recursively down-sampled to form pyramidal feature representations by stride  convolutions, which we denote by $\mathbf{F}_r^{l}$, $\mathbf{F}_{{g}_{1}}^{l}$, $\mathbf{F}_{{g}_{2}}^{l}$, and $\mathbf{F}_{b}^{l}$, where $l=1,2,3$, indexing the pyramid level. Their concatenation form $\mathbf{F}_\text{Intra}^{l}$. We use deformable convolutions instead of plain convolutions for intra-spectral feature representation, so as to learn the convolution support for each instance from its context, expanding the receptive field flexibly. More importantly, we use deformable convolutions to achieve edge-preserving down-sampling.

Features in $\mathbf{F}_\text{Intra}^{1}$ are fused to obtain the inter-spectral feature tensor $\mathbf{F}_\text{Inter}^{1}$ by a sequence of MobileNetV3 convolutions, as it can effectively reduce model complexity with minimal performance loss. 

We aggregate the inter-spectral features under the guidance of an intra-spectral feature matching correlation array, via the local Transformer attention. Taking the red spectrum guidance as an example, at the base level $l=1$, $\mathbf{F}_\text{Inter}^{1}$ and $\mathbf{F}_r^{1}$ are partitioned to non-overlapping windows of spatial size $M\times M$. The feature tensors of the $i$-th window are flattened and transposed, denoted as $\mathbf{F}_\text{Inter}^{(1,i)}$ and $\mathbf{F}_\text{r}^{(1,i)}$. Two linear transformations project $\mathbf{F}_\text{r}^{(1,i)}$ to the \textit{Query} and \textit{Key}, and a linear transformation project $\mathbf{F}_\text{Inter}^{(1,i)}$ to \textit{Value} of the Transformer attention mechanism. In our work, each inter-spectral subband generates two transformation heads. The aggregated features further go through a feed forward residual block, then is down-scaled by a stride convolution, obtaining higher pyramidal-level feature representation $\mathbf{F}_\text{Inter}^{2}$. The top pyramidal level feature $\mathbf{F}_\text{Inter}^{3}$ is computed from $\mathbf{F}_\text{Inter}^{2}$ similarly.

==> method_r.tex <==
\section{Proposed Method}
\label{sec:method}
\subsection{Framework Overview}
\begin{figure*}[htb]
\begin{center}
\includegraphics[width=1\linewidth]{figs/Network.png}
\end{center}
   \caption{The overall architecture of our model. The Bayer image is first rearranged to four channels. The sub-branch generates intra-spectral features to guide the backbone mix inter-spectral features.}
\label{fig:Network}
\end{figure*}
% Let $\mathbf{Y}$ be an RGB image captured by a tri-color sensor on a $2H\times 2W$ lattice $\mathcal{L}$. $\mathbf{Y}$ is composed of samples of the red, green and blue spectra $\mathbf{r}(\mathcal{L})$, $\mathbf{g}(\mathcal{L})$, and $\mathbf{b}(\mathcal{L})$. Let $\mathbf{X}$ be $\mathbf{Y}$'s corresponding CFA image captured by a Bayer sensor. Define subset $\mathcal{R}\in \mathcal{L}$ to collect the positions where the red values are captured, and define $\mathcal{G}$ and $\mathcal{B}$ similarly. $\mathcal{G}$ is further split to $\mathcal{G}_1$ and $\mathcal{G}_2$, which exclusively contain positions at the odd and even rows. We train a deep neural model $f_{\theta}(\mathbf{X})$ parameterized by $\theta$ to estimate $\mathbf{Y}$. 
Briefly, our end-to-end trainable model $f_{\theta}(\mathbf{X})$ takes the form of hierarchical UNet encoder-decoder. It is composed of: an intra-spectral feature generator, an encoder-decoder, and a predictor. Fig.~\ref{fig:Network} depicts our model architecture.

\subsection{Edge-Respecting Feature Generator} 
As described in Sec.~\ref{sec:motivation}, the input $\mathbf{X}$ is first reshaped to $\mathbf{X}_\text{rggb} \in \mathbb{R}^{\mathbf{H}\times\mathbf{W}\times 4}$. That is, neighbouring samples in each $2\times 2$ super-pixel of $\mathbf{X}$: $\mathbf{r}\mathrm(x,y)$, $\mathbf{g}\mathrm{(x,y+1)}$, $\mathbf{g}\mathrm{(x+1,y)}$, $\mathbf{b}\mathrm{(x+1,y+1)}$, are aligned to form a token in $\mathbf{X}_\text{rggb}$ at position $(\lfloor{\frac{\mathrm{x}}{2}\rfloor}+1, \lfloor{\frac{\mathrm{y}}{2}\rfloor}+1)$, for $\mathrm{x}=1,3,\cdots,2\mathrm{H}-1; \mathrm{y}=1,3,\cdots,2\mathrm{W}-1$. Existing demosaicking neural models commonly apply 3D convolutions immediately to $\mathbf{X}_\text{rggb}$. It is barely noticed that, the 3D convolution rests on the premise that all elements of a token have the same neighbourhood. This is equivalent to assuming that all elements in the same super-pixel have the same neighbourhood. Nevertheless, this assumption breaks down at the presence of object boundaries, where the samples in a super-pixel may belong to different objects, and hence having different semantic neighbourhoods. To learn the semantically adaptive neighbourhood for each sample, our model first applies deformable convolutions to each channel (i.e., spectrum) of $\mathbf{X}_\text{rggb}$. We implement it by a residual grouped deformable convolution, followed by a Gaussian Error Linear Unit (GELU) \cite{2016gelu}. The obtained feature tensor $\mathbf{F}_\text{rggb}\in \mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C}}$ is a concatenation of intra-spectral features. Formally, the process of obtaining intra-spectral feature embedding is expressed by:
\begin{align}
    \mathbf{F}_\text{intra} = &\mu \circ c_\text{intra}\left(\mathbf{X}_\text{rggb}\right),
    % \\\nonumber
    % \mathbf{G}_{\mathrm{i}} = &\mu \circ c\left(\mathbf{G}_{\mathrm{i}-1};\theta_{\mathbf{G}_\mathrm{i}}\right)+\mathbf{G}_{\mathrm{i}-1}, \text{for } \mathrm{i} = 1, 2, 3,
\end{align}
where $\mu$ and $c_\text{intra}$ stand for the GELU activation and grouped deformable convolution functions parameterized by $\theta_\text{intra}$; The symbel ``$\circ$'' denotes function composition.

$\mathbf{F}_\text{intra}$ is then transformed to inter-channel feature representation $\mathbf{F}_\text{inter}\in \mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C}}$ by a 3D residual convolution.
\begin{equation}
    \mathbf{F}_\text{inter} = \mu\circ n \circ c_\text{inter}\left(\mathbf{F}_\text{intra}\right)+\mathbf{F}_\text{intra},
\end{equation}
where $n$ means the Layer Normalization function \cite{2016layerNorm}. We set $\mathrm{C}$ to be 64.

\subsection{Pyramidal Encoder-Decoder} 
\label{sec:pyramid}
$\mathbf{F}_\text{inter}$ goes into an U-shaped symmetrical pyramid Encoder-Decoder module with multi-scales. The core components for the encoder-decoder are Diffusion-Fusion blocks and Local Self-Attention Transformer Units.

\textbf{Diffusion-Fusion Block.} We deepen and enhance spectral feature aggregation by the Diffusion-Fusion Module. Among separable convolution methods, we choose Residual Local-UniFormer as the basic building unit for our Diffusion-Fusion module. A Local UniFormer Unit contains a residual depthwise convolution, a MobileNetV2 convolution, and a pair of expanding-shrinking pointwise convolutions. The expanding pointwise convolution enlarges the variety of weighting and combining the spectral information of each token. This process diffuses inter-spectral information to higher dimensional space. The subsequent GELU activation suppresses the non-informative combination schemes for each token. Then the retained elements are projected back to the original dimensional space by a shrinking pointwise convolution. This fuses the inter-spectral information. 

Mathematically, we index each pyramidal level by $\mathrm{L}$, according to their activation order in the data flow. Let $\mathbf{F}_{\mathrm{L},0}$ denote the input feature tensor to the $\mathrm{L}$-th level. The Diffusion-Fusion module cascades $\mathrm{m}_\mathrm{L}$ Local UniFormers, which are denoted by $h_{\mathrm{L},\mathrm{i}}$ for $\mathrm{i}=1, 2, \cdots, \mathrm{m}_\mathrm{L}$, as expressed by
\begin{align}
    \mathbf{F}_{\mathrm{L},\mathrm{i}} = h_{\mathrm{L},\mathrm{i}}(\mathbf{F}_{\mathrm{L},\mathrm{i-1}}) + \mathbf{F}_{\mathrm{L},\mathrm{i-1}}.
\end{align}


% The Diffusion-Fusion module aims at enhancing spectral feature aggregation. As discussed in Sec.~\ref{sec:motivation}, its design follows three principles: 1) separating depthwise and pointwise convolutions; 2) deepening pointwise convolutions; 3) expanding each token to higher dimensional space to generate more proposals for combining inter-spectral representations, then gating the combination proposals and re-projecting them back to the original dimension. Recent separable convolution techniques MobileNet, ConvNeXt, and Local Uniformer meet these principles. In this work, we choose Local Uniformer as the builing uint for our Diffusion-Fusion module.
% should comprises depthwise convolutions and pointwise convolutions, with an emphasis on the pointwise convolutions. The depthwise convolution acts as a local context extractor. The pointwise convolution mixes the inter-spectral information in each token. More importantly, by expanding the tokens to higher dimensional space, our model first diffuses the inter-spectral information in each token to new feature channels. Then a GELU layer performs a gating operation. The gated inter-spectral information are then fused, by a linear projection back to the original low dimensional space. 

\textbf{Local Window Transformer Unit.} The Local Transformer Unit aims at effective spatial feature aggregation. It partitions the spatial dimension of its input feature tensor to $\mathrm{M}\times\mathrm{M}$ non-overlapping windows. In each window, leveraging the self-attention mechanism, pair-wise feature affinity is computed and used to steer the spatial aggregation of tokens. It's worth noting that we do not use global transformers or shifted window transformers in our model because we observe modelling local context dependencies is adequate for demosaicking. This greatly reduces memory consumption.

Mathematically, denote the Local Window Transformer by function $\tau_\mathrm{L}$, the spatial-varying weighted combination is expressed by
\begin{align}
    \mathbf{F}_{\mathrm{L}} = \tau_{\mathrm{L}}(\mathbf{F}_{\mathrm{L},\mathrm{m}_\mathrm{L}}) + \mathbf{F}_{\mathrm{L},\mathrm{m}_\mathrm{L}}.
\end{align}
In particular, $\tau_{\mathrm{L}}$ is a composition of function layers
\begin{align}
    \tau_{\mathrm{L}} = r\circ c_\text{pw}\circ\mu\circ c_\text{pw}\circ{r}\circ{a}\circ{n}\left(\mathbf{F}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\right),
\end{align}
where function $a$ means a Multi-Head Self-Attention Transformer Unit. Specifically, define
\begin{align}
    \tilde{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}} = n\left(\mathbf{F}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\right),
\end{align}
we flatten and transpose each window of $\tilde{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}$ to a feature $\tilde{\mathbf{F}}^\mathrm{(j)}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\in\mathbb{R}^\mathrm{M^2\times C_{L}}$, for $\mathrm{j} = 1, 2, \cdots, \mathrm{\frac{H\times W}{M^2}}$. We then stack these window features to form feature tensor $\bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}$ in the form of 
\begin{align}
    \bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}} = \left[\begin{array}{c}
         \tilde{\mathbf{F}}^\mathrm{(1)}_{\mathrm{L},\mathrm{m}_\mathrm{L}}  \\
         \tilde{\mathbf{F}}^\mathrm{(2)}_{\mathrm{L},\mathrm{m}_\mathrm{L}} \\
         \vdots\\
         \tilde{\mathbf{F}}^\mathrm{(\frac{H\times W}{M^2})}_{\mathrm{L},\mathrm{m}_\mathrm{L}}
    \end{array}\right].
\end{align}
For each head $\mathrm{h}$, the model learns a set of query, key and value transformation matrices $\mathbf{W}^\mathrm{(h)}_{Q}$, $\mathbf{W}^\mathrm{(h)}_K$ and $\mathbf{W}^\mathrm{(h)}_{V}$, which transform $\bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}$ to $\mathbf{Q}$, $\mathbf{K}$ and $\mathbf{V}$, all in $\mathbb{R}^{\mathrm{M}^2\times \mathrm{d}}$ by
\begin{align}
    \mathbf{Q}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\mathbf{W}^\mathrm{(h)}_{Q}, \\\nonumber
    \mathbf{K}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\mathbf{W}^\mathrm{(h)}_{K}, \\\nonumber
    \mathbf{V}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}}\mathbf{W}^\mathrm{(h)}_{V}.
\end{align}
Based on these transformations, the similarity between local query-key pairs guides the aggregation of values by
\begin{align}
\hat{\mathbf{F}}^\mathrm{(h)}_{\mathrm{L},\mathrm{m}_\mathrm{L}} &= \left[\begin{array}{c}
         \hat{\mathbf{F}}^\mathrm{(h,1)}_{\mathrm{L},\mathrm{m}_\mathrm{L}}  \\
         \hat{\mathbf{F}}^\mathrm{(h,2)}_{\mathrm{L},\mathrm{m}_\mathrm{L}} \\
         \vdots\\
         \hat{\mathbf{F}}^\mathrm{(h,\frac{H\times W}{M^2})}_{\mathrm{L},\mathrm{m}_\mathrm{L}}
    \end{array}\right]\\\nonumber
    &=\text{SoftMax}(\frac{\mathbf{Q}^\mathrm{(h)}(\mathbf{K}^\mathrm{(h)})^{T}}{\sqrt{d}}+\mathbf{B})\mathbf{V}^\mathrm{(h)},
\end{align}
where B is the relative position bias\cite{2018Self,2021Swin,2021Uformer}. We then reshape $
\hat{\mathbf{F}}^\mathrm{(h)}_{\mathrm{L},\mathrm{m}_\mathrm{L}}$ to the space $\mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C_L}}$. Finally the Multi-head Self-Attention function $a(\tilde{\mathbf{F}}_{\mathrm{L},\mathrm{m}_\mathrm{L}})$ is a linear projection of the concatenation of outputs from all heads. 

\textbf{Multi-Scale Feature Extraction.} To construct the feature pyramid, we employ $2\times 2$ stride-2 convolutions for down-sampling, and $2\times 2$ stride-2 transposed-convolution for up-sampling. Let $c_\text{sample}$ be the corresponding convolution function, $\mathbf{F}_\mathrm{L+1,0}$ and $\mathbf{F}_\mathrm{L}$ are connected by
\begin{align}
    \mathbf{F}_\mathrm{1,0} & = \mathbf{F}_\text{inter}, \\\nonumber
    \mathbf{F}_\mathrm{L,0} & = c_\text{sample}(\mathbf{F}_\mathrm{L-1}), \text{for } L>1.
\end{align}

\textbf{Hyper-Parameter Setting.} In this work, we set the number of scales to be 3, hence $\mathrm{L}=5$. For $\mathrm{L}\in \left[1,5\right]$, $\mathrm{m_L}$ is set to $\left[6,2,0,2,6\right]$; $\mathrm{C_L}$ set to $\left[64,192,256,192,256\right]$. The dimension expansion rate $\mathrm{r}$ is 4 for all Diffusion-Fusion blocks, and the number of heads for MSA is $8$ for all levels.

\subsection{Warm-Start Predictor} 
A long skip connection sums up $\mathbf{F}_1$ with the decoder output $\mathbf{D}_1$, for the stability of training. The obtained feature map, denoted by $\mathbf{F}_2$, goes into the final predictor, which consists of a 3D convolution layer, a warm-start residual summation layer, and a pixel shuffle layer, to obtain the demosaicked image $f_{\theta}(\mathbf{X})$. The warm-start expands the input CFA image $\mathbf{X}$ to 12 channels, by duplicating the four subbands $\mathbf{r}(\mathcal{R})$, $\mathbf{g}(\mathcal{G}_1)$, $\mathbf{g}(\mathcal{G}_2)$ and $\mathbf{b}(\mathcal{B})$. This tensor, denoted by $\mathbf{W}$, provides the Nearest Neighbour initialization for demosaicking. 
% The base level intra-spectrum feature tensors are further recursively down-sampled to form pyramidal feature representations by stride  convolutions, which we denote by $\mathbf{F}_r^{l}$, $\mathbf{F}_{{g}_{1}}^{l}$, $\mathbf{F}_{{g}_{2}}^{l}$, and $\mathbf{F}_{b}^{l}$, where $l=1,2,3$, indexing the pyramid level. Their concatenation form $\mathbf{F}_\text{Intra}^{l}$. We use deformable convolutions instead of plain convolutions for intra-spectral feature representation, so as to learn the convolution support for each instance from its context, expanding the receptive field flexibly. More importantly, we use deformable convolutions to achieve edge-preserving down-sampling. 

% Features in $\mathbf{F}_\text{Intra}^{1}$ are fused to obtain the inter-spectral feature tensor $\mathbf{F}_\text{Inter}^{1}$ by a sequence of MobileNetV3 convolutions, as it can effectively reduce model complexity with minimal performance loss. 

% We aggregate the inter-spectral features under the guidance of an intra-spectral feature matching correlation array, via the local Transformer attention. Taking the red spectrum guidance as an example, at the base level $l=1$, $\mathbf{F}_\text{Inter}^{1}$ and $\mathbf{F}_r^{1}$ are partitioned to non-overlapping windows of spatial size $M\times M$. The feature tensors of the $i$-th window are flattened and transposed, denoted as $\mathbf{F}_\text{Inter}^{(1,i)}$ and $\mathbf{F}_\text{r}^{(1,i)}$. Two linear transformations project $\mathbf{F}_\text{r}^{(1,i)}$ to the \textit{Query} and \textit{Key}, and a linear transformation project $\mathbf{F}_\text{Inter}^{(1,i)}$ to \textit{Value} of the Transformer attention mechanism. In our work, each inter-spectral subband generates two transformation heads. The aggregated features further go through a feed forward residual block, then is down-scaled by a stride convolution, obtaining higher pyramidal-level feature representation $\mathbf{F}_\text{Inter}^{2}$. We adopt multi-head attention with relative positional encoding \cite{2018Self}, to embed distance affinity into the feature aggregation. The top pyramidal level feature $\mathbf{F}_\text{Inter}^{3}$ is computed from $\mathbf{F}_\text{Inter}^{2}$ similarly.
% In this section, we first explain the architecture of the proposed network. Then we present the blocks involved in detail.
% \subsection{Overall Architecture}
% The overview of the network architecture is illustrated in Figure \ref{fig:Network}. The model is designed to be a U-shaped hierarchical structure, including three main components: Local-UniFormer SE Module (RLUM), SE Deformable Convolution Block (SEDC) and Intra Attention Block (IAB). More details about these components will be given in the following subsections. Except for a encoder-decoder module, our network possessed a sub-branch dedicated to extracting intra-spectral features. A degraded bayer image $I_{bayer}\in\mathbb{R}^{3\times2H\times2W}$ is firstly resampled to $I_{0}\in\mathbb{R}^{4\times H\times W}$ by extracting $2\times2$ patches from $I_{bayer}$ and packs them as a 4 channel feature map.

% Unlike other works, our network performs group-wise convolutions on $I_{0}$ to generate intra-spectral features before the feature maps are fed to the encoder, where the feature maps are divided into 4 parts.
% Next, we perform a $3\times3$ convolution on the grouped feature maps to generate inter-spectral features $I_m \in \mathbb{R}^{C^1\times H\times W}$. Then the feature maps are passed through two encoder layers. We use $2\times2$ convolution with stride 2 to down sample the features. The \emph{l}-th layer produces feature maps $X_{l}\in \mathbb{R}^{C_{l}\times\frac{H}{2^{l}}\times\frac{W}{2^{l}}}$. The first two layers are possessed of a RLUM and a IAB, capable of producing mixed features under the guidance of intra-spectral features from the sub-branch. At the top of the pyramid, we use IAB to learn large-scale dependencies. It's worth noting that we don't use global transformers or shifted window transformers in our model because local context dependencies are adequate for demosaicking, which greatly reduces memory consumption.

% In the decoder stages, each layer has a RLUM and a LeWin self attention block after concatenating the corresponding feature maps from encoder by skip-connection. We use $2\times2$ transposed convolution with stride 2 to up sample the features.

% At the end of the decoder, we add a residual connection with $I_m$ to maintain the expression ability of the network. Inspired by \cite{2018ICPR}, we also apply a residual connection with $I_0$ before up-sampling the features to $2H\times2W$, where $I_0$ is duplicated and reordered to match the RGB sequence and the channel number. We use pixel shuffle to perform the final up-sampling operation and to obtain the restored image.

\subsection{Training Objective} 
To train the parameters of $f_{\theta}$, our training objective combines a Multi-Scale SSIM (MS-SSIM) loss term and an $l_1$-norm loss term between $f_{\theta}(\mathbf{X})$ and the ground truth $\mathbf{Y}$, to preserve the contrast in high-frequency regions \cite{loss},
\begin{equation}
    L =  \alpha \cdot G_{\sigma^M_G} \cdot \norm{f_{\theta}(\mathbf{X})-\mathbf{Y}}_{1}+(1-\alpha) \cdot L_\text{MS-SSIM}(f_{\theta}(\mathbf{X})-\mathbf{Y}),
\end{equation}
where $G_{\sigma^M_G}$ is a Gaussian smoothing functions with standard deviation $\sigma^M_G = 8$; $\alpha$ is set to 0.16. We refer to \cite{loss} for the definition of MS-SSIM loss function $L_\text{MS-SSIM}$.



% \subsection{Residual Local-UniFormer Module}
% We use Local-UniFormer blocks\cite{2022Uniformer}, \emph{i.e.} a generic extension of MobileNetV3 block\cite{2018mobilenetv2}, together with residual connections in the middle and lower layers of the network. Local-UniFormer blocks are capable of capturing local token affinity with static parameter matrices in layers where the receptive field is small. By replacing the self-attention blocks in the shallow layers, RLUM is conductive to reducing redundant computation cost without losing local representations.
%\subsection{SE Deformable Convolution}
%The proposed SEDC block is designed to halve the channel number of the concatenated feature maps. As is shown in Figure \ref{fig:Network}, a SEDC consists of a SE block\cite{2018squeeze} and a $3\times3$ deformable convolution. By utilizing the excitation mechanism, the current channel-wise features and that from the corresponding encoder layer can be weighed together, amplifying the important ones for the sake of better integration. Specifically, $X_{l}^{'} \in \mathbb{R}^{2C_{l}\times\frac{H}{2^{l}}\times\frac{W}{2^{l}}}$ is firstly excited and then convolved adaptively, halving its channel number at the same time.
% \subsection{Intra-spectral Sub-branch}
% In order to utilize intra-spectral information, we design a sub-branch dedicated to mining intra dependencies by performing group-wise operations. For Bayer image demosaicking, the group number is always set to 4, \emph{i.e.} RGGB. The sub-branch also adopts a hierarchical structure to match the resolution of the encoder stages and the top of the U-shaped backbone. At the bottom of the sub-branch, also the head of the network, we use $3\times3$ group convolution blocks with residual connections to obtain grouped features $I_{RGGB}^0\in \mathbb{R}^{C_0\times H \times W}$. In the rest part of the sub-branch, the network doesn't do other operations other than down-sampling.

% We use $2\times2$ group deformable convolution with stride 2 to down sample each group and expand the number of channels to match the corresponding features in the network backbone.
%---------------------------------------------------------
\begin{table*}[htb]
\centering
\caption{Quantitative comparison against state-of-the-art works on image demosaicking. Best and second-best results are \textbf{highlighted} and {\ul underlined}, respectively. The ’-’ represents that the results are not provided by the corresponding paper.}
%\setlength{\tabcolsep}{3mm}{
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Params(M)} & \multicolumn{2}{c|}{McMaster}                       & \multicolumn{2}{c|}{Kodak}                          & \multicolumn{2}{c|}{CBSD68}                           & \multicolumn{2}{c|}{Urban100}                         \\ \cline{3-10} 
                        &                            & \multicolumn{1}{c|}{PSNR}           & SSIM            & \multicolumn{1}{c|}{PSNR}           & SSIM            & \multicolumn{1}{c|}{PSNR}           & SSIM            & \multicolumn{1}{c|}{PSNR}           & SSIM            \\ \hline
Mosaic                  & -                          & \multicolumn{1}{c|}{9.17}           & 0.1674          & \multicolumn{1}{c|}{8.56}           & 0.0682          & \multicolumn{1}{c|}{8.43}           & 0.0850          & \multicolumn{1}{c|}{7.48}           & 0.1195          \\
IRCNN                   & 0.19                       & \multicolumn{1}{c|}{37.47}          & 0.9615          & \multicolumn{1}{c|}{40.41}          & 0.9807          & \multicolumn{1}{c|}{39.96}          & 0.9850          & \multicolumn{1}{c|}{36.64}          & 0.9743          \\
NTSDCN                  & -                          & \multicolumn{1}{c|}{39.48}          & -               & \multicolumn{1}{c|}{42.79}          & -               & \multicolumn{1}{c|}{-}              & -               & \multicolumn{1}{c|}{-}              & -               \\
RNAN                    & 8.96                       & \multicolumn{1}{c|}{39.71}          & 0.9725          & \multicolumn{1}{c|}{43.09}          & 0.9902          & \multicolumn{1}{c|}{{\ul 42.50}}    & {\ul 0.9929}    & \multicolumn{1}{c|}{39.75}          & 0.9848          \\
DAGL                    & 5.62                       & \multicolumn{1}{c|}{{\ul 39.84}}    & {\ul 0.9735}    & \multicolumn{1}{c|}{{\ul 43.21}}    & {\ul 0.9910} & \multicolumn{1}{c|}{\textbf{-}}     & \textbf{-}      & \multicolumn{1}{c|}{\textbf{40.20}} & {\ul 0.9854}    \\
(Ours)                  & 5.85                       & \multicolumn{1}{c|}{\textbf{40.14}} & \textbf{0.9885} & \multicolumn{1}{c|}{\textbf{43.29}} & {\textbf{0.9958}}    & \multicolumn{1}{c|}{\textbf{42.83}} & \textbf{0.9962} & \multicolumn{1}{c|}{{\ul 40.17}}    & \textbf{0.9919} \\ \hline
\end{tabular}
}
\label{tbl:DM}
\end{table*}
%---------------------------------------------------------

% \subsection{Intra Attention Block}
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=1\linewidth]{figs/IAB.png}
% \end{center}
%    \caption{(left) Intra Attention Block. (right) Multi-Head Cross Attention consists of several attention layers running in parallel. Each group of RGGB generates QK for h heads.}
% \label{fig:IAB}
% \end{figure}
% In most other transformer-based architectures, the network only uses multi-head self attention blocks for image restoration. It's unfavorable to utilize other guidance information. To address the problem and make transformer operations applicable to high-resolution feature maps, we propose a window transformer block capable of taking advantage of intra-spectral information to capture long-range dependencies. 

% \textbf{Window-based Multi-head Cross-Attention (W-MCA).} A W-MCA block computes cross-attention within non-overlapping local windows as is shwon in Figure \ref{fig:IAB}. Given the mixed feature maps $X_m\in \mathbb{R}^{C\times H\times W}$, and the intra-spectral feature maps $X_{RGGB}\in \mathbb{R}^{C\times H\times W}$, it segments these maps into $M\times M$ non-overlapping windows and then get the flattened and transposed features $X^i_m\in \mathbb{R}^{M^2\times C}$ and $X^{i}_{RGGB}\in \mathbb{R}^{M^2\times C}$.

% Suppose the head number is $K$, the head number of each RGGB group is thus $h=K/4$ and the dimension per head is $d_k=C/K$. For example, the k-th head of group R can be formulated as follows,
% \begin{equation}
%     \begin{split}
%     &X_m = \{X_m^1,X_m^2,\cdot,X_m^N\},\,N=HW/M^2, \\
%     &X_{R} = \{X_{R}^1,X_{R}^2,\cdot,X_{R}^N\},\,N=HW/M^2, \\
%     &Y_k^i = Attention(X_{R}^iW_k^Q,X_{R}^iW_k^K,X_{m}^iW_k^V),\,
%  i=1,\cdot,N,\\
%     &\hat{X}_k = \{Y_k^1,Y_k^2,\cdot,Y_k^N\},
%     \end{split}
% \end{equation}
% where $W_k^Q, W_k^K, W_k^V \in \mathbb{R}^{C\times d_k}$ represent the projection matrices of the queries, keys and values for the k-th head in group R and $\hat{X}_k$ is the output of this head. The outputs of group G1, G2 and B can be obtained in the same way. The attention calculation can be formulated as:
% \begin{equation}
%     Attention(Q,K,V) = SoftMax(\frac{QK^T}{\sqrt{d_k}}+B)V,
% \end{equation}
% where B is the relative position bias\cite{2018Self,2021Swin,2021Uformer}.
% Then the final result of the block is a linear projection of the concatenation of outputs from all heads. 

% It's worth noting that the queries and keys originate from the intra-spectral features while the values come from the mixed features. For each head group of $h=K/4$ heads, our W-MCA block learns the affinity between the mixed features and the intra-spectral features. By fusing the guidance of all 4 groups, we can produce stronger features than traditional self-attention transformers.

==> method_r1.tex <==


\section{Methodology}
\label{sec:method}
This section first outlines the architecture amd workfloe of our model, then details the key building units.

\subsection{Overview}
\label{subsec:overview}
Briefly, our end-to-end trainable model $f_{\theta}(\mathbf{X})$ comprises: an edge-respecting feature generator, a hierarchical U-Shape encoder-decoder, and a predictor. Fig.~\ref{fig:Network} depicts our model architecture. 

\textbf{Edge-Respecting Feature Generator.} From the input Bayer image $\mathbf{X}$, our model first extracts spatially-adaptive intra-spectral feature representation $\mathbf{F}_\text{intra}$, which further generates shallow inter-spectral feature representation $\mathbf{F}_\text{inter}$. 

\textbf{Multi-Scale Feature Encoder-Decoder.} UNet \cite{UNet} has proved effective and been widely adopted in dense prediction tasks (e.g., UFormer \cite{2021Uformer}). We follow this vein, but particularly design the encoding-decoding stages toward Moir\'{e}-free while detail-preserving. Each stage comprises multiple Spectral Communication Enhancing Blocks and one Spatial Detail Sharpening Block. The last decoder stage outputs feature tensor $\mathbf{F}_{\mathrm{d}}$ (subscript ``d'' stands for ``decoding''). 

\textbf{Predictor.} The predictor aims at transforming the $\mathrm{H}\times\mathrm{W}\times\mathrm{C}$ tensor $\mathbf{F}_{\mathrm{D}}$ to an RGB image of size $\mathrm{2H}\times\mathrm{2W}\times\mathrm{3}$. Inspired by \cite{2018ICPR}, our model initializes the prediction from a warm-start, by duplicating the four subbands $\mathbf{r}(\mathcal{R})$, $\mathbf{g}(\mathcal{G}_1)$, $\mathbf{g}(\mathcal{G}_2)$ and $\mathbf{b}(\mathcal{B})$ of $\mathbf{X}$ to form $\mathbf{F}_\text{init}$. It is refined by a residual tensor $\mathbf{F}_\text{r}$, transformed from $\mathbf{F}_{\mathrm{d}}$ via a 3D convolution.

Next we articulate how the proposed model achieves its goals.

% A long skip connection sums up $\mathbf{F}_\text{inter}$ with the decoder output $\mathbf{F}_{\mathrm{2S+1}}$, to bypass gradient vanishing or explosion during training. The obtained feature map $\mathbf{F}_\text{d}$ goes into the final predictor. There, $\mathbf{F}_\text{d}$ is transformed to $\mathbf{F}_\text{r}$ with 12 feature channels by a 3D convolution layer. We then use a Warm-Start Initialization layer to expand the input CFA image $\mathbf{X}$ to 12 channels, denoted by $\mathbf{F}_\text{init}$, by duplicating the four subbands $\mathbf{r}(\mathcal{R})$, $\mathbf{g}(\mathcal{G}_1)$, $\mathbf{g}(\mathcal{G}_2)$ and $\mathbf{b}(\mathcal{B})$. That is, $\mathbf{F}_\text{init}$ provides the Nearest Neighbour initialization for demosaicking as a warm-start. A residual connection sums up $\mathbf{F}_\text{init}$ with $\mathbf{F}_\text{r}$. The summation is then reshaped to a demosaicked image $f_{\theta}(\mathbf{X})$ by pixel-shuffling.
% 
% For spatial up-scaling, our predictor employs the pixel-shuffle technique instead of transposed convolution to avoid the checker-board artifacts. To this end, our model is designed to transform $\mathbf{F}_{\mathrm{2S+1}}$ to an $\mathrm{H}\times\mathrm{W}\times\mathrm{12}$ feature tensor $\mathbf{F}_\text{p}$ (subscript ``p'' for ``pre-shuffle''), then reshapes it to the RGB image $f_{\theta}(\mathbf{X})$. Therefore, we design $\mathbf{F}_{\mathrm{2S+1}}$ to be transformed to a tensor $\mathbf{F}_\text{r}$ (subscript ``r'' for ``residual'')  of size 
% $\mathrm{H}\times\mathrm{W}\times\mathrm{12}$, via a 3D convolution; Then a skip connection sums up $\mathbf{F}_\text{init}$ and $\mathbf{F}_\text{r}$ to generate the pre-shuffle feature tensor $\mathbf{F}_\text{p}$.

\subsection{Edge-Respecting Feature Generator} 
As described in Sec.~\ref{sec:motivation}, the input $\mathbf{X}$ is first reshaped to $\mathbf{X}_\text{rggb} \in \mathbb{R}^{\mathbf{H}\times\mathbf{W}\times 4}$. That is, neighbouring samples $\mathbf{r}\mathrm(x,y)$, $\mathbf{g}\mathrm{(x,y+1)}$, $\mathbf{g}\mathrm{(x+1,y)}$, $\mathbf{b}\mathrm{(x+1,y+1)}$ of $\mathbf{X}$, for $\mathrm{x}=1,3,\cdots,2\mathrm{H}-1; \mathrm{y}=1,3,\cdots,2\mathrm{W}-1$, are aligned to form a token in $\mathbf{X}_\text{rggb}$ at position $(\lfloor{\frac{\mathrm{x}}{2}\rfloor}+1, \lfloor{\frac{\mathrm{y}}{2}\rfloor}+1)$. Existing demosaicking neural models commonly apply 3D convolutions immediately to $\mathbf{X}_\text{rggb}$. It is barely noticed that, however, the 3D convolution rests on the premise that all elements of a token have the same neighbourhood. Nevertheless, this assumption breaks down at the presence of object boundaries, where neighbouring samples may belong to different objects, thus having different semantic neighbourhoods. To learn the semantically adaptive neighbourhood for each sample, our model first applies deformable convolutions \cite{2017Deformable} to each channel (i.e., spectrum) of $\mathbf{X}_\text{rggb}$. 

We generate the edge-respecting features by a layer of 2D grouped deformable convolutions $c_\text{intra}$, followed by a Layer Normalization (LN) \cite{2016layerNorm} function $n$, and a Gaussian Error Linear Unit (GELU) \cite{2016gelu} $\mu$. The obtained feature tensor $\mathbf{F}_\text{intra}\in \mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C}}$ is a concatenation of intra-spectral features. Formally, the process is expressed by:
\begin{align}
    \mathbf{F}_\text{intra} = &\mu\circ n \circ c_\text{intra}\left(\mathbf{X}_\text{rggb}\right),
    % \\\nonumber
    % \mathbf{G}_{\mathrm{i}} = &\mu \circ c\left(\mathbf{G}_{\mathrm{i}-1};\theta_{\mathbf{G}_\mathrm{i}}\right)+\mathbf{G}_{\mathrm{i}-1}, \text{for } \mathrm{i} = 1, 2, 3,
\end{align}
where symbol ``$\circ$'' denotes function composition.

$\mathbf{F}_\text{intra}$ is then transformed to inter-channel feature representation $\mathbf{F}_\text{inter}\in \mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C}}$ by a 3D convolution $c_\text{inter}$, followed by a Local Spatial Detail Sharpener Module $a_\text{L-Spatial}$, i.e.,
%followed by Windowed Multi-Heads Self-Attention (W-MSA) transformation $a_\text{W-MSA}$ (see Sec.~\ref{sec:detail} for computation details), i.e.,
\begin{equation}
    \mathbf{F}_\text{inter} = a_\text{Spatial}\circ\mu\circ n \circ c_\text{inter}\left(\mathbf{F}_\text{intra}\right).
\end{equation}

\textbf{Demosaicking with or without Denoising.} Demosaicking has been studied in two scenarios: Joint Demosaicking-Denoising and Independent Demosaicking. Research works on joint demosaicking-denoising models generally assume that the noise follows the additve white Gaussian distribution, whose standard deviation is estimated from the CFA image. At the training stage, a random noise map, which is sampled at a range of parameters, is input to the network together with noise contaminated $\mathbf{X}$; At the inference stage, the random noise map is sampled with a given distribution parameter. 

For joint demosaicking-denoising, we follow the literature to simulate additive white Gaussian noise contamination on the Bayer input $\mathbf{X}$, and attach a noise map with $\mathbf{X}$. We concatenate the noise map with each of the four subbands of $\mathbf{X}_\text{rggb}$, to perform 2D grouped deformable convolutions. Our noise sampling routine is as same as previous works for training and inference.  

\textbf{Hyper-Parameter Settings.} In the feature generator, we set $\mathrm{C}$ to 64, the window size to $8\times 8$, and the total number of heads for self-attention to 8.  

\subsection{Multi-Scale Feature Encoder-Decoder}
\label{sec:MFED}
$\mathbf{F}_\text{inter}$ goes into a multi-scale U-Shaped symmetrical Encoder-Decoder. The feature pyramid has $\mathrm{S}$ scales, each of which containing an encoding block and a decoding block of the same structure, except the coarsest scale, which acts as a bottleneck. We index these blocks by $\mathrm{b}=1, 2, \cdots, \mathrm{2S}-1$, according to their execution order in the workflow. To construct the feature pyramid, we employ $2\times 2$ stride-2 convolutions for down-sampling, and $2\times 2$ stride-2 transposed-convolution for up-sampling. Let $c_\text{sample}$ be the corresponding convolution function, and the output of the $\mathrm{b}$-th block be $\mathbf{F}_\mathrm{b}$. The input $\mathbf{F}_\mathrm{b,0}$ to the $(\mathrm{b}+1)$-th block is obtained by: 
\begin{align}
\label{eq:stage}
    \mathbf{F}_\mathrm{1,0} & = \mathbf{F}_\text{inter}, \\\nonumber
    \mathbf{F}_\mathrm{b+1,0} & = c_\text{DownSample}(\mathbf{F}_\mathrm{b}), \text{for }  \mathrm{b \in [1, S-1]}, \nonumber\\
    \mathbf{F}_\mathrm{b+1,0} & = c_\text{UpSample}(\mathbf{F}_\mathrm{b})^\frown\mathbf{F}_\mathrm{2S-b}, \text{for }  \mathrm{b \in [S, 2S-2], }
\end{align}
where symbol ``$^\frown$'' indicates the concatenation operation.

Each encoding or decoding block is composed of $\mathrm{m_b}$ Spectral Communication Enhancer modules and one Spatial Detail Sharpener module, described as below.

\textbf{Spectral Comminication Enhancer Module.} Our strategy to achieve cross-spectral consistency is to enhance information exchanging in the spectral-dimension. To this end, 
we separate spatial and spectral feature representations, and deepen spectral feature extraction by adding point-wise convolutions. Moreover, inspired by the expansion-reversion technique used in separable convolution networks such as MobileNet, ConvneXt, and Uniformer, we adapt the added point-wise convolutions to diffuse, weight, then fuse the high-order spectral responses. 

Particularly, a Spectral Consistency Enhancer module starts from a residual depth-wise convolution, which extracts local spatial contexts. Then a separable convolution MobileNetV3 building unit is adapted to perform weighted combination of the spatial filtering response maps. Then a point-wise convolution linearly projects the feature to a four times higher dimensional space. This operation proposes a large variety of schemes to weight and combine spectral information of each token, thus diffusing inter-spectral information to a higher dimensional space. There we use the Squeeze-Excitation channel attention mechanism to gate these proposals, and a subsequent GELU activation suppresses the non-informative combination schemes for each token. Finally the GELU retained elements are projected back to the original dimension by a reversion point-wise convolution. This fuses the inter-spectral information selectively. 

In terms of function composition, denote the Spectral Consistency Enhancer module function by $h_{\mathrm{b},\mathrm{i}}$ for $\mathrm{i}=1, 2, \cdots, \mathrm{m}_\mathrm{b}$, they are cascaded by
\begin{align}
    \mathbf{F}_{\mathrm{b},\mathrm{i}} = h_{\mathrm{b},\mathrm{i}}(\mathbf{F}_{\mathrm{b},\mathrm{i-1}}) + \mathbf{F}_{\mathrm{b},\mathrm{i-1}}, \text{for } \mathrm{i}\geq 1,
\end{align}
where $\mathbf{F}_{\mathrm{b},0}$ is defined as in Eq.~\ref{eq:stage}.

Without loss of generality, function $h$ (omitting subscripts $\mathrm{b}$ and $\mathrm{i}$) is expressed by 
\begin{align}
    h=c_\text{dw}\circ c_\text{pw}\circ c_\text{dw}\circ c_\text{pw}\circ n\circ c_\text{ex} \circ a_\text{SE}\circ\mu\circ c_\text{re},
\end{align}
where $c_\text{ex}$ and $c_\text{re}$ are the dimension expansion and reversion linear projections.

\textbf{Spatial Detail Sharpener Module.} Each founding block of our encoder-decoder ends with a Spatial Detail Sharpener Module, which aims at effective spatial feature aggregation, hence employs Local Window Self-Attention. It partitions the spatial dimension of its input feature tensor to $\mathrm{M}\times\mathrm{M}$ non-overlapping windows. In each window, leveraging the self-attention mechanism, pair-wise feature affinity is computed and used to steer the spatial aggregation of tokens. It's worth noting that we do not use global transformers or shifted window transformers in our model because we observed that modelling local context dependencies is adequate for demosaicking, while greatly reducing memory consumption.

%Mathematically, denote the Local Window Transformer by function $\tau_\mathrm{b}$, the spatial-varying weighted combination is expressed by
The spatial-varying weighted combination is formulated by
\begin{align}
    \mathbf{F}_{\mathrm{b}} = a_\text{MSA}(\mathbf{F}_{\mathrm{b},\mathrm{m}_\mathrm{b}}) + \mathbf{F}_{\mathrm{b},\mathrm{m}_\mathrm{b}}.
\end{align}
% In particular, $\tau$ (omitting the subscript $\mathrm{b}$) is a composition of function layers
% \begin{align}
%     \tau = \circ{r}\circ{a_\text{MSA}}\circ{n},
% \end{align}
where function $a_\text{MSA}$ means a Multi-Head Self-Attention transformation, which is implemented as follows. Define
\begin{align}
    \tilde{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}} = n\left(\mathbf{F}_{\mathrm{b},\mathrm{m}_\mathrm{b}}\right),
\end{align}
% we flatten and transpose each window of $\tilde{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}$ to a feature $\tilde{\mathbf{F}}^\mathrm{(j)}_{\mathrm{b},\mathrm{m}_\mathrm{b}}\in\mathbb{R}^\mathrm{M^2\times C_{b}}$, for $\mathrm{j} = 1, 2, \cdots, \mathrm{\frac{H\times W}{M^2}}$. We then stack these window features to form feature tensor $\bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}$ in the form of 
% \begin{align}
%     \bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}} = \left[\begin{array}{c}
%          \tilde{\mathbf{F}}^\mathrm{(1)}_{\mathrm{b},\mathrm{m}_\mathrm{b}}  \\
%          \tilde{\mathbf{F}}^\mathrm{(2)}_{\mathrm{b},\mathrm{m}_\mathrm{b}} \\
%          \vdots\\
%          \tilde{\mathbf{F}}^\mathrm{(\frac{H\times W}{M^2})}_{\mathrm{b},\mathrm{m}_\mathrm{b}}
%     \end{array}\right].
% \end{align}
% For each head $\mathrm{h}$, the model learns a set of query, key and value transformation matrices $\mathbf{W}^\mathrm{(h)}_{Q}$, $\mathbf{W}^\mathrm{(h)}_K$ and $\mathbf{W}^\mathrm{(h)}_{V}$, which transform $\bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}$ to $\mathbf{Q}$, $\mathbf{K}$ and $\mathbf{V}$, all in $\mathbb{R}^{\mathrm{M}^2\times \mathrm{d}}$ by
% \begin{align}
%     \mathbf{Q}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}\mathbf{W}^\mathrm{(h)}_{Q}, \\\nonumber
%     \mathbf{K}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}\mathbf{W}^\mathrm{(h)}_{K}, \\\nonumber
%     \mathbf{V}^\mathrm{(h)} &= \bar{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}}\mathbf{W}^\mathrm{(h)}_{V}.
% \end{align}
% Based on these transformations, the similarity between local query-key pairs guides the aggregation of values by
% \begin{align}
% \hat{\mathbf{F}}^\mathrm{(h)}_{\mathrm{b},\mathrm{m}_\mathrm{b}} &= \left[\begin{array}{c}
%          \hat{\mathbf{F}}^\mathrm{(h,1)}_{\mathrm{b},\mathrm{m}_\mathrm{b}}  \\
%          \hat{\mathbf{F}}^\mathrm{(h,2)}_{\mathrm{b},\mathrm{m}_\mathrm{b}} \\
%          \vdots\\
%          \hat{\mathbf{F}}^\mathrm{(h,\frac{H\times W}{M^2})}_{\mathrm{b},\mathrm{m}_\mathrm{b}}
%     \end{array}\right]\\\nonumber
%     &=\text{SoftMax}(\frac{\mathbf{Q}^\mathrm{(h)}(\mathbf{K}^\mathrm{(h)})^{T}}{\sqrt{d}}+\mathbf{B})\mathbf{V}^\mathrm{(h)},
% \end{align}
% where B is the relative position bias\cite{2018Self,2021Swin,2021Uformer}. We then reshape $
% \hat{\mathbf{F}}^\mathrm{(h)}_{\mathrm{b},\mathrm{m}_\mathrm{b}}$ to the space $\mathbb{R}^{\mathrm{H}\times\mathrm{W}\times\mathrm{C_b}}$. Finally the Multi-head Self-Attention function $a(\tilde{\mathbf{F}}_{\mathrm{b},\mathrm{m}_\mathrm{b}})$ is a linear projection of the concatenation of outputs from all heads. 

\textbf{Hyper-Parameter Setting.} We set the number of scales to be 3, hence our model has 5 encoding and decoding blocks. For $\mathrm{b}\in \left[1,5\right]$, $\mathrm{m_b}$ is set to $\left[6,2,0,2,6\right]$; $\mathrm{C_b}$ is set to $\left[64,192,256,192,64\right]$. Uniformly in all modules, the dimension expansion rate $\mathrm{r}$ is 4, and the number of heads for MSA is $8$ with window size $8\times8$.

\subsection{Warm-Start Predictor} 
 A long skip connection sums up $\mathbf{F}_\text{inter}$ with the decoder output $\mathbf{F}_{\mathrm{2S-1}}$, to avoid gradient vanishing or explosion. The obtained feature map $\mathbf{F}_\text{d}$ (subscript ``d'' for decoding), i.e., 
  \begin{align}
     \mathbf{F}_{\mathrm{d}} = \mathbf{F}_\text{inter}+\mathbf{F}_{\mathrm{2S-1}},
 \end{align}
 goes into the final predictor. 
 
 The predictor should up-scale the feature spatial resolution from $\mathrm{H}\times\mathrm{W}$ to $\mathrm{2H}\times\mathrm2{W}$. To bypass the checker-board artifacts suffered by de-convolution \cite{odena2016deconvolution}, here we employ the pixel-shuffle technique for up-scaling \cite{shi2016real}. This requires our model to predict a pre-shuffle tensor $\mathbf{F}_\text{p}$ of size $\mathrm{H}\times\mathrm{W}\times\mathrm{12}$ (subscript ``p'' for ``pre-shuffle'') from $\mathbf{F}_{\text{d}}$. Moreover, we initialize $\mathbf{F}_\text{p}$ by a warm-start $\mathbf{F}_\text{init}$, which duplicates the channels of $\mathbf{X}_\text{rggb}$ to 12 channels by 
 \begin{align}
     \mathbf{F}_\text{init} = \text{concat}\left[\right.\begin{array}{cccc}
         \mathbf{r}(\mathcal{R}), & \mathbf{r}(\mathcal{R}), & \mathbf{r}(\mathcal{R}), & \mathbf{r}(\mathcal{R}),\\
         \mathbf{g}(\mathcal{G}_1), &\mathbf{g}(\mathcal{G}_1), &\mathbf{g}(\mathcal{G}_2), &\mathbf{g}(\mathcal{G}_2),\\
         \mathbf{b}(\mathcal{B}), &\mathbf{b}(\mathcal{B}), &\mathbf{b}(\mathcal{B}), &\mathbf{b}(\mathcal{B})
     \end{array}\left.\right]
 \end{align}

 Given these design considerations, $\mathbf{F}_\text{d}$ is designed to generate the refinement tensor $\mathbf{F}_\text{r}$ (subscript ``r'' for ``refinement'') on top of $\mathbf{F}_\text{init}$, via a W-MSA transformation and a 3D convolution layer. Formally, the predictor is formulated as,
 \begin{align}
     \mathbf{F}_\text{r} &= c_\text{3D}\circ a_\text{W-MSA}(\mathbf{F}_\text{d}),\\\nonumber
     \mathbf{F}_\text{p} &= \mathbf{F}_\text{r}+\mathbf{F}_\text{init},\\\nonumber
     f_{\theta}(\mathbf{X}) &= \text{PixelShuffle}(\mathbf{F}_\text{p}).
 \end{align}

\subsection{Training Objective} 
To train the parameters of $f_{\theta}$, we adopt the training objective suggested by  \cite{loss} for its robustness to outliers. In particular, it is defined as a weighted combination of the $l_1$-norm distance between $f_{\theta}(\mathbf{X})$ and the ground truth $\mathbf{Y}$ and a Multi-Scale Structural Similarity (MS-SSIM) loss term. 
\begin{align}
    L =  &\alpha \cdot G_{\sigma^M_G} \cdot \norm{f_{\theta}(\mathbf{X})-\mathbf{Y}}_{1}\\\nonumber
    &+(1-\alpha) \cdot L_\text{MS-SSIM}(f_{\theta}(\mathbf{X})-\mathbf{Y}),
\end{align}
where $G_{\sigma^M_G}$ is a set of Gaussian kernels with standard deviations $\sigma^M_G = \left[0.5,~1.0,~2.0,~4.0,~8.0\right]$; Weight $\alpha$ is set to 0.16. We refer readers to \cite{loss} for the definition of MS-SSIM loss function $L_\text{MS-SSIM}$.

\subsection{Implementation Details}
\label{sec:detail}
\textbf{W-MSA Computation.} Particularly, the W-MSA function $a_\text{W-MSA}(\mathbf{F})$ of a general tensor $\mathbf{F}$ is computed as follows. We partition the $\mathrm{H}\times\mathrm{W}$ grid into $\mathrm{M}\times\mathrm{M}$ windows, each of which is flattened and transposed to $\tilde{\mathbf{F}}^\mathrm{(j)}\in\mathbb{R}^\mathrm{M^2\times C}$, for $\mathrm{j} = 1, 2, \cdots, \mathrm{\frac{H\times W}{M^2}}$. We then stack them to form a tensor $\bar{\mathbf{F}}$ in the form of 
\begin{align}
    \bar{\mathbf{F}} = \left[\begin{array}{c}
         \tilde{\mathbf{F}}^\mathrm{(1)}  \\
         \tilde{\mathbf{F}}^\mathrm{(2)} \\
         \vdots\\
         \tilde{\mathbf{F}}^\mathrm{(\frac{H\times W}{M^2})}
    \end{array}\right].
\end{align}
For each head $\mathrm{h}$, the model learns a set of query, key and value transformation matrices $\mathbf{W}^\mathrm{(h)}_{Q}$, $\mathbf{W}^\mathrm{(h)}_K$ and $\mathbf{W}^\mathrm{(h)}_{V}$, which transform $\bar{\mathbf{F}}$ to $\mathbf{Q}^\mathrm{(h)}$, $\mathbf{K}^\mathrm{(h)}$ and $\mathbf{V}^\mathrm{(h)}$, all in $\mathbb{R}^{\mathrm{M}^2\times \mathrm{d}}$ by
\begin{align}
    \mathbf{Q}^\mathrm{(h)} &= \bar{\mathbf{F}}\mathbf{W}^\mathrm{(h)}_{Q}, \\\nonumber
    \mathbf{K}^\mathrm{(h)} &= \bar{\mathbf{F}}\mathbf{W}^\mathrm{(h)}_{K}, \\\nonumber
    \mathbf{V}^\mathrm{(h)} &= \bar{\mathbf{F}}\mathbf{W}^\mathrm{(h)}_{V}.
\end{align}
Then the similarity between local Query-Key pairs guides the aggregation of Values by
\begin{align}
\hat{\mathbf{F}}^\mathrm{(h)} =\text{SoftMax}(\frac{\mathbf{Q}^\mathrm{(h)}(\mathbf{K}^\mathrm{(h)})^{T}}{\sqrt{d}}+\mathbf{B})\mathbf{V}^\mathrm{(h)},
\end{align}
% \begin{align}
% \hat{\mathbf{F}}^\mathrm{(h)}_{\mathrm{b},\mathrm{m}_\mathrm{b}} &= \left[\begin{array}{c}
%          \hat{\mathbf{F}}^\mathrm{(h,1)}_{\mathrm{b},\mathrm{m}_\mathrm{b}}  \\
%          \hat{\mathbf{F}}^\mathrm{(h,2)}_{\mathrm{b},\mathrm{m}_\mathrm{b}} \\
%          \vdots\\
%          \hat{\mathbf{F}}^\mathrm{(h,\frac{H\times W}{M^2})}_{\mathrm{b},\mathrm{m}_\mathrm{b}}
%     \end{array}\right]\\\nonumber
%     &=\text{SoftMax}(\frac{\mathbf{Q}^\mathrm{(h)}(\mathbf{K}^\mathrm{(h)})^{T}}{\sqrt{d}}+\mathbf{B})\mathbf{V}^\mathrm{(h)},
% \end{align}
where $\mathbf{B}$ is the relative position bias \cite{2018Self,2021Swin,2021Uformer}. We then reshape each row of $\hat{\mathbf{F}}^\mathrm{(h)}$ back to $\mathrm{M}\times\mathrm{M}\times{\mathrm{d}}$ windows, forming a feature tensor $\tilde{\mathbf{F}}^\mathrm{(h)}$. Finally the concatenation of the outputs from all heads are linearly projected, obtaining $a_\text{W-MSA}(\mathbf{F})$.

\textbf{Training Details.} Following previous works, we use DIV2K\cite{2017NTIRE} dataset for training. The training samples are augmented by random rotations of 90$^\circ$, 180$^\circ$, 270$^\circ$, and horizontally flipping. Each mini-batch contains 32 Bayer patches of size 64$\times$64. Our model is trained using the AdamW optimizer \cite{2017AdamW} with $\beta_1=0.9$, $\beta_2=0.999$, and a weight decay rate of 0.05. Initialized by 2e-4, the learning rate is recursively halved every 200 epochs. We observe that 1200 epochs are sufficient for the training process to converge.









==> motivation.tex <==
\section{Problem Statement and Motivation}
\label{sec:motivation}

Let $\mathbf{Y}$ be an RGB image captured by a tri-color sensor on a $2\mathrm{H}\times 2\mathrm{W}$ lattice $\mathcal{L}$. $\mathbf{Y}$ is composed of samples of the red, green and blue spectra $\mathbf{r}(\mathcal{L})$, $\mathbf{g}(\mathcal{L})$, and $\mathbf{b}(\mathcal{L})$. Let $\mathbf{X}$ be $\mathbf{Y}$'s corresponding CFA image captured by a CFA sensor. To simplify description, here we take Bayer CFA as an example, as in most previous works. Define subsets $\mathcal{R},~\mathcal{G},~\mathcal{B}$ of $\mathcal{L}$ to collect the positions where the red, green and blue values are captured. $\mathcal{G}$ is further split to $\mathcal{G}_1$ and $\mathcal{G}_2$, which exclusively contain positions at the odd and even rows. We train a deep neural model $f_{\theta}(\mathbf{X})$ to estimate $\mathbf{Y}$, where $\theta$ indicates all learnable parameters. 

A particular issue for demosaicking, is that samples of different spectra are interleaved in each neighbourhood in the CFA image $\mathbf{X}$. Directly applying plain convolutions to $\mathbf{X}$ would cause misinterpretation of the color context. A popular solution is to decompose $\mathbf{X}$ into four subbands $\mathbf{r}(\mathcal{R})$, $\mathbf{g}(\mathcal{G}_1)$, $\mathbf{g}(\mathcal{G}_2)$ and $\mathbf{b}(\mathcal{B})$, then concatenate them as feature channels to form a tensor $\mathbf{F}_{0}\in\mathbb{R}^{\mathrm{H}\times \mathrm{W}\times 4}$ before convolution\footnote{There are other solutions for feature embedding, for example, Bilinearly interpolating the CFA image to an RGB image. But same as reordering, all spectra in these solutions are concatenated along the third dimension to form a feature tensor. So their feature dimension is also the spectral dimension.}. Suppose we are to extract features from $\mathbf{F}_{0}$ by a kernel of size ${\mathrm{k}\times \mathrm{k}\times 4}$, whose four planes are $\mathbf{k}^{(\mathrm{i})}, \mathrm{i} = 1, 2, 3, 4$, then the convolution can be written as the summation of four 2D spatial convolutions
\begin{align}
\label{eq:spectral}
    \mathbf{F}_{1}^{(1)} = &\mathbf{k}^{(1)}\circledast \mathbf{r}(\mathcal{R})+\mathbf{k}^{(2)}\circledast \mathbf{g}(\mathcal{G}_{1})+\mathbf{k}^{(3)}\circledast \mathbf{g}(\mathcal{G}_{2})
    + \mathbf{k}^{(4)}\circledast \mathbf{b}(\mathcal{B}),
\end{align}
where symbol $\circledast$ stands for convolution. Clearly, $\mathbf{F}_{1}^{(1)}$ is an inter-spectral summation of the local spatial information in each spectrum. The kernel may degenerate to intra-channel convolution (i.e., only one kernel of these $\mathbf{k}^{(\mathrm{i})}$ contains non-zero coefficients), if learned from data. Recursively, further convolution on $\mathbf{F}_\mathrm{l}$ yields higher-order inter-spectral aggregation $\mathbf{F}_{\mathrm{j}+1}$ for $\mathrm{j}\geq 1$. Thus for demosaicking problem, the feature dimension is physically the ``spectral dimension''. This is different from other image restoration problems, the feature channels of which do not have the spectral distinction.  

Therefore, to obtain high frequency consistency across spectra, the key is to \textit{enhance spectral convolutions rather than spatial convolutions}. Barely noticing this, existing demosaicking CNN models widely adopt 3D convolutions as for other image restoration tasks. However, the 3D convolution binds spectral processing and spatial processing together. Therefore deepening spectral processing would also deepen spatial processing, leading to over-wide receptive field, which further causes ambiguity for demosaicking, a task can be well solved from local context. 

Motivated by the above analysis, we propose unbinding the spectral and spatial aggregations. Particularly, we design a spectral diffusion-fusion module to exchange high frequency context across spectra. We also integrate it with restricted number of local Self-Attention Transformations to steer spatial feature aggregation by feature edges.
% Although any intra-spectral spatial interpolation can generate an estimate to the RGB image from the CFA image, the lack of inter-spectral regularization would cause the ``false color'' or ``moir\'e'' artifacts \cite{szeliski2010}. Thus the key to demosaicking is to accurately infer the missing values from their spatial-spectral (local or non-local) context. It can be modeled by mathematically expressed priors (e.g., \cite{HA96, HQLI04, MLRI16, NiuTIP2019, ni2020color}), or be learned from data by Random Fields \cite{MSR2014}, Compressive Sensing \cite{LDSR14}, Dictionary Learning \cite{DDR16}, Convolutional Neural Networks (CNN) \cite{MNN14}, etc. In recent years, deep CNN models, which can learn the spatial-spectral correlation among high semantic level features, have attracted significant research attention in the field of demosaicking. 

% Some CNN-based demosaicking models treat the three color channels equally to generate inter-spectral features \cite{DJ16, MDFCN18, CAS18, chen2021Wild}, and some guide the restoration of the red and blue channels by the intermediately restored green channel \cite{2Stage17, 3Stage18, liu2020SG, 2020NTSDCN}. There are also works exploiting the cross-spectra correlation by converting the RGB restoration to color difference restoration \cite{yan2019channel, elgendy2021low}. To fuse the inter-spectral features spatially adaptively, Liu et al. proposed weighting the inter-spectral features by local contrast of the intermediately estimated green channel \cite{liu2020SG}; Zhang et al. proposed generating the parameters of spatially varying convolution kernels from the CFA pattern \cite{zhang2022deep}. So far the effective application of Transformer \cite{2020ViT} to demosacking has barely been discussed.

% Another related line of work is Image Restoration neural models, some of which cover demosaicking as a general dense interpolation problem (e.g., IRCNN \cite{2017IRCNN}, RNAN \cite{2019RNAN}, DAGL \cite{2021DAGL}). A few recent image restoration algorithms also explore the superiority of Transformer over traditional convolutions (e.g., Uformer \cite{2021Uformer}, Restormer \cite{2022restormer}). However, these methods focus on modelling the long range spatial correlation of the features rather than the spectral-spatial correlation.

% Different from existing works, we use local Transformer to exploit the spatial-spectral feature correlation, which is the central problem of demosaicking. 
